Optimal Sorting Circuits for Short Keys

A long-standing open question in the algorithms and complexity literature is whether there exist sorting circuits of size $o(n \log n)$. A recent work by Asharov, Lin, and Shi (SODA'21) showed that if the elements to be sorted have short keys whose length $k = o(\log n)$, then one can indeed overcome the $n\log n$ barrier for sorting circuits, by leveraging non-comparison-based techniques. More specifically, Asharov et al.~showed that there exist $O(n) \cdot \min(k, \log n)$-sized sorting circuits for $k$-bit keys, ignoring $poly\log^*$ factors. Interestingly, the recent works by Farhadi et al. (STOC'19) and Asharov et al. (SODA'21) also showed that the above result is essentially optimal for every key length $k$, assuming that the famous Li-Li network coding conjecture holds. Note also that proving any {\it unconditional} super-linear circuit lower bound for a wide class of problems is beyond the reach of current techniques. Unfortunately, the approach taken by Asharov et al.~to achieve optimality in size somewhat crucially relies on sacrificing the depth: specifically, their circuit is super-{\it poly}logarithmic in depth even for 1-bit keys. Asharov et al.~phrase it as an open question how to achieve optimality both in size and depth. In this paper, we close this important gap in our understanding. We construct a sorting circuit of size $O(n) \cdot \min(k, \log n)$ (ignoring $poly\log^*$ terms) and depth $O(\log n)$. To achieve this, our approach departs significantly from the prior works. Our result can be viewed as a generalization of the landmark result by Ajtai, Koml\'os, and Szemer\'edi (STOC'83), simultaneously in terms of size and depth. Specifically, for $k = o(\log n)$, we achieve asymptotical improvements in size over the AKS sorting circuit, while preserving optimality in depth.

==> Makefile <==
# Switched this back to bibtex because the current version of crosstex
# seems to have a bug causing incorrect capitalization in the titles.

LATEX=pdflatex
TEXFLAGS=

TARGET=para-osort-smallkey.pdf 

all: $(TARGET)

$(TARGET): $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
#	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
#	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
#	$(LATEX) $(TEXFLAGS) $<


full: $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	

test: test-fonts test-info

test-fonts: $(TARGET)
	pdffonts $<

test-info: $(TARGET)
	pdfinfo $<

print: $(TARGET)
	pdftops $< - | lpr -P lws510

view: $(TARGET)
	kpdf $<

clean:
	rm -f $(TARGET) *.log *.aux *.bbl *.blg *.out *.bak .*.xtx.cache parsetab.py \#*\# *~


==> circuit-model.tex <==
% !TEX root = compaction-circuit.tex

\subsection{Background: the Circuit Model of Computation}
\label{sec:circuitmodel}

We briefly review the circuit model of computation,
following the presentation of Asharov, Lin, and Shi~\cite{soda21}.
We use an operational model in which we allow 
generalized boolean gates of constant fan-in and constant fan-out
implementing any truth table between the inputs and outputs, and
we define selector gates which are used to move the 
payload strings around.



%\subsection{Circuit Model of Computation}

\paragraph{Circuit model of computation.}
We adopt the standard boolean circuit model of computation~\cite{savagebook}.
A boolean circuit consists of AND, OR, and NOT gates. Gates 
are connected through wires. 
Each gate's output can be fed into $O(1)$ number of other gates as input. 
All the gates and their wires form a directed acyclic graph.
By definition, such a boolean circuit has constant fan-in and constant fan-out.
A circuit's size is the number of gates 
the circuit contains.

%\subsection{Operational Model Used in Our Paper}
\paragraph{Operational model used in this paper.}
For convenience, we use the following operational model for circuits when describing
our algorithms.
In our operational model, we allow the following
gadgets in our circuitry: 1) constant-sized %fan-in, constant fan-out  
gadgets that implement an arbitrary truth table between the $O(1)$ input 
bits and the $O(1)$ output bits; and 2) selector gates.
When defining our circuits we will count explicitly how many generalized boolean gates the circuit has, and how many selector and reverse selectors are there. 
We give more explanations below and describe how to convert a circuit in our operational model 
to a standard boolean circuit with constant fan-in and constant fan-out.

\begin{itemize}[leftmargin=5mm,itemsep=1pt]
\item 
{\it Selector and reverse selector gates.}
A $w$-selector gate  (``MUX'') takes in one bit $b$ and two input elements $m_0,m_1$
each of bit-width $w$, and outputs $m_b$.
Each $w$-selector gate can be realized with 
$C \cdot w$ number of AND, OR, and NOT gates where $C > 1$ is a universal constant.

Reverse selector gates are the opposite. A $w$-reverse selector 
gate takes one 
element $m$ of bit-width $w$ and a signal $b \in \{0, 1\}$ as input and 
outputs $(m,0^w)$ if $b=0$ and $(0^w,m)$ if $b=1$. 

Henceforth in the paper whenever we count 
selector and reverse selector gates, we do not distinguish between them and count
both towards selector gates. 

\item 
{\it Generalized boolean gates.}
Generalized boolean gates are allowed to have constant fan-in and constant fan-out.
Without loss of generality, we allow 
each generalized boolean gate to implement {\it any truth table}
between the $O(1)$ input bits to the $O(1)$ output bits. 
Realizing such a generalized boolean gate 
with AND, OR, and NOT gates 
will only incur an $O(1)$ factor blowup in the circuit's size.
Later in our paper, we will use 
generalized boolean gates of fan-in at most 3 and fan-out at most
3. %\elaine{adjust these constants in the end. they need to be universal constants} 

\end{itemize}

\ignore{
\paragraph{Unbounded fan-out is free.}
From standard complexity theory textbooks~\cite{savagebook}, we
know that constant fan-in, unbounded fan-out circuits of size $G(n)$  
can be converted to constant fan-in, constant fan-out 
circuits of size $O(G(n))$. \elaine{double check the precise statement}
Therefore, in our operational model, we 
allow the output of a gate to be fed into unbounded number of gates.
\elaine{TO FIX: this conversion can cost in depth}
}

\elaine{TO DO: check where unbounded fan-out was 
used in earlier paper, we cannot use it in this paper.}


\begin{remark}[Selector gates and indivisibility model]
Our construction uses selector gates to move payloads 
around, and our construction does not perform 
any boolean computation or encoding of the payloads.
This also means that our construction works in the 
{\it indivisibility} model.
In some works~\cite{isthereoramlb,osortsmallkey}, the indivisibility 
model is also referred
to as the {\it balls-and-bins} model, i.e., each element's payload
string behaves like an opaque, indivisible ball. 

Given a circuit in the indivisibility model, 
one construct a mirroring circuit in the \emph{reverse order}
where selector gates are converted to reverse-selector gates, and this reverse
circuit can route the payloads back into their initial positions.
Our construction later will make use of such ``reverse routing''.
\end{remark}








==> fix-errors.tex <==
% !TEX root = para-osort-smallkey.tex

\section{Fix Errors}

\weikai{
(SlowSort) To sort $m$ elements of at most $K$ keys in $O(mK)$ work and $O(\log m)$ depth:\\
1. duplicate $m$ elements into $K$ lists, $L_1,\dots, L_K$.\\
2. for each list $L_i$, count the number of key $i$ in $L_i$ and let $c_i$ be the resulting count.\\
3. for each $j\in[K]$, let $s_j = 1 + \sum_{i=1}^{j-1} c_i$ be the starting point of key $j$.\\
4. for each list $L_i$, route all key $i$ to locations $s_i+1, s_i+2, \dots, s_i+c_i$, let $L'_i$ be the results.\\
5. multiplex $K$ lists of $L'_i$ into the output list.
}

\weikai{
To compute majority of $m$ elements of at most $K$ keys in $O(m)$ work and $O(\log K + \log m)$ depth:\\
1. divide into $m/5$ groups, each group consists of $5$ elements.\\
2. find the majorities of each group.\\
3. recursively call this procedure on the majorities until the number of elements is $m/K^2$,
that is $2k = \log K^2$ recursive calls.\\
4. perform SlowSort on $m/K^2$ elements.\\
5. output the $(m/2K^2)$th element in the sorted list.
}


\weikai{use segment for continuous, subarray for non-cont}

Given $p\in\N$, consider a sorted array $\hat A$ with partition $\hat P = (\hat A_1,\dots, \hat A_p)$
such that $\hat A = \hat A_1 \| \dots \| \hat A_p$ 
and $\abs{\hat A_i} = \abs{\hat A_{i'}}$ for all $i,i'\in[p]$.
We say a segment $\hat A_i$ is \emph{single-keyed} if and only if
all elements in $\hat A_i$ have the same key,
or \emph{multi-keyed} otherwise.
Suppose that $\hat A$ consists of at most $K$ distinct keys.
Then, as $\hat A$ is sorted,
there are at most $K-1$ ``transitions''
(where a transition is defined as an element in $\hat A$
such that its succeeding element has a distinct key).
Because segment $\hat A_i$ is single-keyed if and only if $\hat A_i$ has no transition,
for any integers $p, K$, there are at most $K-1$ multi-keyed segments
and at least $p - K + 1$ single-keyed segments in $\hat P$.

Let $\eta \in (0,1/2)$ be a fixed fraction.
We further suppose that $\hat A$ is a sorted array of $A$,
where $A = A_1\|\dots\| A_p$ is $(\eta,p)$-orderly with partition $P=(A_1,\dots, A_p)$.
Given only $(A,P)$ (but not $\hat A$ nor $\hat P$),
imagine that we know in advance for each $i$,
whether $\hat A_i$ is single-keyed or multi-keyed.
As $A$ is $(\eta,p)$-orderly and $\eta < 1/2$,
using the imaginary information, we know that for each single-keyed $\hat A_i$,
the majority elements $\maj(A_i)$ are all in correct locations
(and we call such elements are \emph{correct}).
To fully sort $A$, it suffices to permute incorrect elements
while keeping the correct elements unmoved.
That is, it suffices to move all incorrect elements to a leftover array,
sort the leftover array, and then move the elements from 
the sorted leftover array back to $A$.
However, such sorting relies on the imaginary information 
(i.e., whether a segment $\hat A_i$ is single-keyed),
which is defined by the sorted array $\hat A$, and thus such procedure seems circular.
In this section, our key idea is to efficiently identify
the indices of all single-keyed segments from $(A,P)$
without fully sorting $A$ so that the circularity is avoided.


\subsection{Good and Bad Segments}
Suppose an array $A$ with partition $P=(A_1,\dots, A_p)$ is $(\eta,p)$-orderly.
As a one-sided estimation of single- or multi-keyed segments,
we define a segment $P$ is $\good$ or $\bad$ as below.
\begin{quote}
For each segment $A_i$, we say $A_i$ is $\good$ if and only if $A_i$ is $(1- \eta)$-uniform.
Otherwise, we say $A_i$ is $\bad$.
\end{quote}
Recall that $\hat A$ is a sorted array of $A$ and that $\hat A$ is partitioned into
$\hat P = (\hat A_1,\dots, \hat A_p)$.
By the definition of $(\eta,p)$-orderly, if $\hat A_i$ is single-keyed, then $A_i$ must be $\good$.
The converse does not hold:
if $\hat A_i$ is multi-keyed, then $A_i$ can still be good
as a simple result of having a majority in $\hat A_i$.
Using {\bf FindDominant} algorithm (Theorem~\ref{}),
it is straightforward to identify each segment $A_i$ is good or bad.

\begin{mdframed} 
\underline{$\textsf{GoodSegment}_{\eta}(A_i)$}
\begin{enumerate}
\item 
Perform ${\bf FindDominant}(A_i, K, \abs{A_i})$, let $m$ be the outcome.
\item 
Count the number of $m$ in $A_i$, let $c$ be the count.
\item 
Output ``no'' if $c < (1- \eta)\cdot\abs{A_i}$;
otherwise output ``yes'' and the dominant key $m$.
\end{enumerate}
\end{mdframed}

\weikai{to fill theorem}

\paragraph{Just ``good'' is not enough.}
In each good segment $A_i$, there are at least $(1 - \eta)$ fraction of majority elements.
It is tempting to think that such $(1 - \eta)$ fraction of elements are all in correct locations,
but this is false.
For example, let $\hat A_i \in \hat P$ be a multi-keyed segment
but there is an $\eta' > \eta$ fraction differ from the majority, and the errors of $(\eta,p)$-orderly
introduced some more majority elements into $A_i$ so that the corresponding $A_i$
consists of $(1- \eta)$-fraction majority elements and is classified as good.

In such example,
we should move some majority elements out of $A_i$ to fully sort $A$,
yet we do not know which or how many should be moved.
Hence, in the next subsection,
we solve this challenge and obtain a full sorting.
% we identify whether a good segment is really single-keyed.

% We stress that if $\hat A_i$ is multi-valued then $A_i$ must be bad,
% but if $\hat A_i$ is single-valued then $A_i$ can be
% either good or bad.
% Given only the $\epsilon$-sorted partition of $A$,
% we next compute whether each $\hat A_i$ is single- or multi-valued
% as a step toward obtaining the fully sorted result.

% \weikai{To elaborate on why just good/bad is not yet straightforward:
% as a good piece can be multi-valued,
% such piece could ``shift'' the elements to other pieces in a long range
% and then broke correctness on many other good pieces.
% Our next subsection is a constructive proof
% showing that does not happen.
% }

% \subsection{Identify Single-Keyed Segments}

% \weikai{simplification: 
% no need counting, just let the threshold of ``Good'' be $\tau$,
% and for each Good moves $2 \tau$ out, where $\tau$ is the guarantee of errro fraction}

% Given an $(\tau,p)$-orderly array $A$ with respect to 
% partition $P = (A_1,\dots, A_p)$,
% we want to label each segment $A_i$ as either single-keyed or multi-keyed.

% To compute such labeling, the idea is simple:
% using $(A,P)$, we can efficiently count 
% the number of occurrence of key $j$ in $A$ for each key $j \in [K]$,
% and then using the counts to label a segment
% is a straightforward comparison.
% It is because for each good segment,
% there is a majority key occupies at least $(1- \tau)$ fraction,
% and we can ``compress'' all majority elements into one element.
% Namely, in the good segment, 
% we count the number of all majority elements,
% replace such elements with one element 
% of the same majority key but attaches the count (i.e., \emph{weighting}).
% Any other elements remain in weighting 1.
% Because each good segment is compressed down by $\tau$ fraction,
% we then fully sort the compressed elements by keys,
% and counting the sorted keys with weighting is simple,
% which yields the desired overall counting of $A$.
% The procedure below describes the remaining details.

% \weikai{all sorting below are performed on a small subset of $A$
% so we simply use the $O(nK)$ work algorithm.}

% \begin{mdframed} 
% \underline{$\SingleKeyedSegment_{\tau,p}(A, P = (A_i, \dots, A_p))$}
% \begin{enumerate}
% \item 
% Duplicate all elements in $(A_1,\dots, A_p)$ into $(B_1,\dots, B_p)$.
% For each $i\in[p]$, perform ${\sf GoodSegment}_\tau(A_i)$,
% let $m_i := \maj(A_i)$ be the majority 
% if ${\sf GoodSegment}_\tau(A_i)$ outputs ${\good}$.

% \item 
% For each good segment $B_i$,
% aggregate the majority elements as:
% \begin{enumerate}
% \item 
% Count the number of $m_i$ in $B_i$, let the number be $c_i$.
% \item 
% For each element $(x,v) \in B_i$ 
%   \begin{itemize}
%   \item 
%   If $x = m_i$, replace the first occurrence with $(x, c_i)$
%   and all other occurrences with $\bot$.
%   \item 
%   If $x \neq m_i$, replace $x$ with $(x, 1)$.
%   \end{itemize}
% \end{enumerate}
% \item 
% For each bad segment $B_i$, for each element $(x,v) \in B_i$,
% replace $x$ with $(x, 1)$.

% \item 
% Perform tight compaction on $B := B_1 \| \dots \| B_p$ so that all $\bot$ are removed.
% Then, sort the the compacted array by the first coordinate 
% and let $B' = \left((x_1, c_1), (x_2, c_2), \dots\right)$ be the result
% (so that $x_i \leq x_j$ for all $i < j$).
% Compute prefix sums on the second coordinate of $B'$,
% i.e., $\left((x_1, s_1), (x_2, s_2), \dots\right)$ where
% $s_i := \sum_{j=1}^{i}c_j$ are the prefix sums.
% Erase non-transition pairs and keep only transition pairs,
% i.e., for each $i$, replace $(x_i,s_i)$ with $\bot$ 
% if and only if $x_i = x_{i+1}$.
% Let the result be $C = \left((x_1, s_1), (x_2, s_2), \dots\right)$
% (where a pair $(x_i, s_i)$ can be $\bot$).

% \item 
% For each $i \in [p]$,
% let $(y_i, t_i)$ be the pair as below.
% % For each segment $A_i$,
% % let $(y_{2i-1}, t_{2i-1})$ and $(y_{2i}, t_{2i})$ be pairs such that 
% \begin{enumerate}
%   \item 
%   Let $t_i$ be the first location of $A_i$,
%   where the location is counted from the beginning of $A$.
%   \item 
%   If $A_i$ is good, then $y_i$ is set to $m_i$.
%   Otherwise, $A_i$ is bad, set $y_i$ to $\bot$
%   (as $A_i$ is always multi-keyed).
% \end{enumerate}
% Let $C' := \big((y_1, t_1), \dots, (y_p, t_p), (y_{p+1}, t_{p+1})\big)$,
% where $(y_{p+1}, t_{p+1}) := (\bot, |A|+1)$.

% \item 
% Sort $C \| C'$ by the second coordinate,
% break tie by putting an $x$-pair after a $y$-pair,
% let $S(C \| C')$ be the sorted array.
% For each $i \in [p]$ such that $A_i$ is $\good$,
% output $A_i$ is single-keyed if and only if in $S(C \| C')$,
% \begin{itemize}
%   \item 
%   there is no $x$-pair between $(y_i, t_i)$ and $(y_{i+1}, t_{i+1})$,
%   or
%   \item 
%   there is exactly one $x$-pair $(u,v)$ between 
%   $(y_i, t_i)$ and $(y_{i+1}, t_{i+1})$ and $v = t_{i+1} - 1$ holds.
% \end{itemize}
% That is, $A_i$ is single-keyed if and only if
% there is no transition between $t_i$ and $t_{i+1}-1$.
% \end{enumerate}
% \end{mdframed}

% \weikai{to add thm state, analysis}

% \weikai{will use this to bound efficiency in this subsection}
% Because the number of multi-keyed segments is at most $K-1$ in $\hat A$,
% we directly have that the number of bad segments is 
% at most $K-1$ in $A$.


\subsection{Fully Correct Sorting}

We rely on following two observations to identify incorrect elements 
in the $(\eta,p)$-orderly partition of $A$.
The first observation is that each single-keyed segment $\hat A_i$ implies a good segment $A_i$
so that we always have at least $p-K+1$ good segments.
The second observation is that, even though a multi-keyed $\hat A_i$ can imply a good $A_i$,
that can only happen when $\hat A_i$ has \emph{at least} $1-2 \eta$ elements are majority
(otherwise, the $\eta$ fraction of errors introduced by the $(\eta,p)$-orderly partition
can not imply $1- \eta$ majority that is identified as good).
Now we can correctly and efficiently sort all elements since the number of bad segments 
and the number of incorrect elements in good segments are both bounded.

We next present the fully correct sorting.
Taking as input an array of $n$ elements each tagged with a $k$-bit key,
the sorting begins with applying the $(2^{-2k}, 2^{2k})$-partial sorter
so that we obtains $(2^{-2k}, 2^{2k})$-orderly segments.
Then, we identify all good segments using ${\sf GoodSegment}$
described in the previous subsection.
There are at least $(1-2 \eta)$ fraction of majority elements in each good segment,
% Each majority element in each single-keyed segment
% is in the correct location,
and all other elements are compacted down to the leftover array.
The leftover array is then sorted using $\SlowSort$,
and it suffices to restore the sorted leftover elements back to
the locations which they compacted from.
The sorting is formally described below.

% We present an algorithm such that 
% for any $n \in \N, k < 0.1 \log n$,
% for any array of $n$ elements each tagged with a $k$-bit key,
% the algorithm sorts the array correctly 
% in $O(n k)$ work and $O(\log n)$ depth.

\begin{mdframed} 
\underline{$\textsf{SortSmallKeys}_{k}(A)$}, 
where $A$ is an array of $n$ elements each has a $k$-bit key.
\begin{enumerate}
\item 
Let $\eta := 2^{-2k}, p := 2^{2k}$, and $K := 2^k$.
Perform the $(\eta,p)$-partial-\splitter on $A$ (Theorem~\ref{}),
let $P = (B_1, \dots, B_p)$ be the result.
% Let $B := B_1 \| \dots \| B_p$.

\item 
For all $i\in[p]$ in parallel, perform ${\sf GoodSegment}_\eta(B_i)$, 
and then mark $A_i$ as $\good$ if ${\sf GoodSegment}$ outputs ``yes''and 
let $m_i$ be the dominant key (otherwise mark $A_i$ as $\bad$ and let $m_i := \bot$).

% \item 
% Perform $\SingleKeyedSegment_{\tau,p}(B,P)$
% so that each $B_i$ is tagged with either 
% single-keyed or multi-keyed.
% For each single-keyed $B_i$, 
% compute $m_i \gets \Majority(B_i)$.

\item 
In parallel, copy $B_i$ into $C_i$ for all $i\in[p]$.
For all $i \in [p]$ in parallel, if $C_i$ is $\good$,
erase exactly $(1-2 \eta)\cdot n/p$ elements tagged with key $m_i$ in $C_i$.

\item 
Perform tight compaction on $C_1 \|\dots\|C_p$
so that the erased elements are in the back,
and let $\leftover$ be the front $n' := 2 \eta n + (2^{-k})n$ elements
where each element is associated with its \emph{originating location} in $C$;
also record all element moves performed 
during the tight compaction into the list $\Aux$.

\item 
For all non-erased elements in $\leftover$,
route the $i$-th smallest element to the $i$-th smallest originating location
(for each $i\in [n']$).
To do so, it suffices to apply $\SlowSort^K$ for three times:
\begin{enumerate}
  \item 
  sort all $\leftover$ by key and yield $\leftover_1$,
  \item 
  sort all originating locations but memorizing the ``current locations''
  and yield $\leftover_2$,
  \item 
  copy elements from $\leftover_1$ to $\leftover_2$ coordinate-wise,
  and finally
  \item 
  sort $\leftover_2$ by the memorized ``current locations'' 
  so that each originating location obtains the desired element.
\end{enumerate}
Let the resulting array be $\leftover'$.
% \weikai{to write SlowSort such that sorts $m$ elements
% in $O(m\cdot 2^k)$ work and $O(\log m)$ depth.}

\item 
Move elements from $\leftover'$ back to $C$ using $\Aux$,
let the resulting array be $C'$.

\item 
For each $j\in[n]$ in parallel, replace the element $B[j]$ with $C'[j]$ 
if and only if $C'[j]$ is not erased, let the result be $B' = B'_1 \|\dots\|B'_p$.
\weikai{to prove $B'$ is $(0,p)$-orderly, which needs to enumerate 4 cases 
of good/bad between 2 adjacent segments}

\item 
Sort elements within each segment $B'_i$ for all $i\in[p]$. This is achieved by:
\begin{enumerate}
  \item 
  For all $i\in[p]$ in parallel, count the number of distinct keys in $B'_i$
  and mark $B'_i$ as multi-keyed when there are more than one keys.
  \item 
  Perform tight compaction so that multi-keyed segments are permuted to the front
  and meanwhile record the movements of all segments into $\Aux'$;
  let the resulting segments be $B'_{i_1},\dots,B'_{i_p}$.
  \item 
  For each $j\in[K]$ in parallel, perform $\SlowSort^K(B'_{i_j})$ and 
  let $\tilde B'_{i_j}$ be the result.
  \item 
  Reverse route segments $\tilde B'_{i_1},\dots,\tilde B'_{i_{K}}, B'_{i_{K+1}}, \dots, B'_{i_p}$
  back using $\Aux'$, let $\O$ be the resulting segments concatenated.
\end{enumerate}

\item 
Output the the array $\O$.
\end{enumerate}
\end{mdframed}


\weikai{
thm state, proof. 
may need a ``claim'' saying it suffices to sort all incorrect elements.
}


==> form.tex <==
A long-standing open question in the algorithms and complexity literature is whether there exist sorting circuits of size $o(n\log n)$. A recent work by Asharov et al.~(SODA'21) showed that if the elements to be sorted have short keys whose length $k=o(\log n)$, then there exist $O(n)\cdot\min(k,\log n)$-sized sorting circuits for $k$-bit keys, ignoring $poly\log^*$ factors. Interestingly, the recent works by Farhadi et al.~(STOC'19) and Asharov et al.~also showed that the above result is essentially optimal for every key length $k$, assuming that the famous Li-Li network coding conjecture holds. Note also that proving any {\it unconditional} super-linear circuit lower bound for a wide class of problems is beyond the reach of current techniques.

Unfortunately, the approach taken by previous works to achieve optimality in size relies on sacrificing the depth. Asharov et al.~phrase it as an open question how to achieve optimality both in size and depth. In this paper, we close this gap and construct a sorting circuit of size $O(n)\cdot\min(k,\log n)$ (ignoring $poly\log^*$ terms) and depth $O(\log n)$. To achieve this, our approach departs significantly from the prior works. Our result can be viewed as a generalization of the landmark result by Ajtai, Koml\'os, and Szemer\'edi (STOC'83), simultaneously in terms of size and depth. Specifically, for $k=o(\log n)$, we achieve asymptotical improvements in size over the AKS sorting circuit, while preserving optimality in depth.


==> oldintro.tex <==
\section{Old Intro: to remove}


To get this main result requires a significant
amount of new machinery.
Along the way, we go through two major stepping stones
that are each of independent interest --- we present them below:
%the main results of the 
%two stepping stones below.

\paragraph{Main result 2: sorting short keys 
on an oblivious PRAM, optimal in work and depth.}
To eventually get our sorting circuit result, 
we first make the problem a little easier by considering 
how to deterministically sort $n$ elements
each with a $k$-bit key on an oblivious Parallel RAM (PRAM). 
A deterministic algorithm 
in the oblivious PRAM model is a PRAM algorithm whose
memory access patterns do not depend on the input 
(except the input size).
We show that indeed, one can obliviously sort 
$n$ elements
each with a $k$-bit key in $O(n) \cdot \min(k, \log n)$ total
work and $O(\log n)$ depth, assuming that each element
can be stored in $O(1)$ memory words.
The total work is optimal assuming either
the indivisibility model or the Li-Li network coding
conjecture~\cite{osortsmallkey,soda21}, and the depth
is optimal unconditionally even for 1-bit keys~\cite{orlbpram}.
%Both the total work 
%and the depth are optimal
%due to known lower bounds~\cite{osortsmallkey,soda21,orlbpram}.
%The total work 
%is optimal for every $k$ due to 
%\elaine{FILL}, and 
%the depth is optimal due to \elaine{FILL}.


\begin{theorem}[Sorting short keys on an oblivious PRAM]
There exists a deterministic oblivious parallel algorithm
that sorts any input array
containing $n$ elements each with a $k$-bit key
in $O(n) \cdot \min(k, \log n)$
total work and $O(\log n)$ depth, assuming that each element
can be stored in $O(1)$ words\footnote{Note that the theorem statement
for oblivious PRAM does {\it not}
 have an extra $\poly\log^*$ blowup in total work.}.
\label{thm:intro-sort-opram}
\end{theorem}
%\elaine{say it's optimal in this model too.}

Prior to our work, it was known that   
$n$ elements with $k$-bit keys 
can sorted by a {\it randomized} oblivious algorithm 
in $O(k n \frac{\log \log n}{\log k})$
work and polylogarithmic depth~\cite{osortsmallkey}.
It is possible to improve the total work to  
$O(k n)$ and get rid of the randomization 
by combining techniques from Lin et al.~\cite{osortsmallkey}
%using new building blocks from 
and Asharov et al.~\cite{paracompact}.
However, to the best of our knowledge, existing techniques 
are stuck at polylogarithmic depth. 
To attain the above result,  
our techniques depart significantly from the prior 
works~\cite{osortsmallkey,soda21}.

More concretely, 
we leverage the linear-work, logarithmic depth oblivious {\it compaction}
algorithm by Asharov et al.~\cite{paracompact}.
Compaction (also called {\it tight compaction})
is a special case of sorting where the key is promised to be 1 bit.
The crux is how to efficiently upgrade 
the 1-bit oblivious sorting 
to $k$-bit oblivious sorting %for $k = o(\log n)$.
incurring only a $k$-factor 
more work relative to the 1-bit case, 
and preserving the depth.
A na\"ive idea for achieving this 
is to rely on Radix sort,
but this fails on multiple accounts:
1) the $1$-bit case 
(i.e., the compaction algorithm) is {\it not stable}, and this
is inherent as mentioned~\cite{lbmult,osortsmallkey};
and 2) using Radix sort would have incurred polylogarithmic depth.
Lin, Shi, and Xie~\cite{osortsmallkey}
and Asharov et al.~\cite{soda21}
proposed a new 2-parameter recursion trick 
to accomplish this upgrade. Their technique overcomes
the non-stability challenge, but 
unfortunately still suffers from polylogarithmic depth.

We propose a fundamentally different approach to accomplish the 1-bit
to $k$-bit upgrade.  
Specifically, we define a new building block
called a {\it nearly orderly segmenter}.
A nearly orderly segmenter 
partially sorts the input array 
taking $O(nk)$ work and $O(\log n)$ depth, 
such that if we divide the outcome into $2^{3k}$ segments, 
each segment contains at most $1/2^{-8k}$ 
fraction of elements that do not belong in the segment.
We then propose a novel algorithm that 
uses oblivious compaction~\cite{paracompact} and 
additional new building blocks to detect and correct the 
remaining errors in 
linear work and logarithmic depth.
Note that our nearly ordered segmenter is 
comparator-based, but the second step that corrects
the remaining errors relies on non-comparison-based techniques  
(for example, the oblivious compaction building block 
itself is non-comparison-based).

%If it were stable, we could have used well-known techniques
%such as Radix sort for the upgrade (although in fact Radix
%\elaine{this solves an open question of our earlier soda paper, this
%result is of independent interest}


%getting our circuit result requires 
%significant additional techniques.

\paragraph{Main result 3: linear-sized, logarithmic 
depth compaction circuit.}
We stress that the above {\it oblivious PRAM result does not directly give 
our circuit result} and vice versa.
%As we will show later, 
%It turns out that getting a result in the circuit model
%is even more non-trivial.
It turns out that 
going from our oblivious PRAM result to our circuit result
is highly non-trivial.
The reason is that in a PRAM model, the word size is at least $\log n$ bits
and one can perform arithmetic and boolean 
operations on $\log n$ bits in {\it unit cost}.
Indeed, by leveraging this capability, a recent work~\cite{paracompact}
relied on the so-called ``packing'' technique to 
achieve an optimal oblivious parallel compaction
algorithm. Specifically, they showed that sorting $n$ elements  
each with a 1-bit key can be accomplished 
in $O(n)$ work and $O(\log n)$ depth on an oblivious PRAM.
Unfortunately, in the circuit model,
there is no more free lunch and 
operations on $\log n$ bits incur logarithmic or more cost.
As a result, 
%an the counterpart of this in the circuit model 
a compaction circuit optimal in both size and depth is not known.
The work by Asharov et al.~\cite{soda21}
showed how to achieve optimality in 
circuit size for compaction (modulo $\poly\log^*$ factors), 
but at the price of 
%as mentioned, their compaction circuit suffers from 
super-{\it poly}logarithmic depth.

We fill in this gap and show how to construct a compaction circuit
optimal in both size and depth (barring an extra $\poly\log^*$ factor 
in size), as stated in the following theorem:

\begin{theorem}[Linear-sized, logarithmic-depth tight compaction circuit]
There is a circuit of size $O(nw) \cdot \max(\poly(\log^* n - \log^* w), 1)$
and depth $O(\log n + \log w)$ 
that can sort any array containing elements with 1-bit keys
and $w$-bit payloads.
%generalized boolean gates,
%$O(n) \cdot \max(\poly\log^* n - \poly\log^* w, 1)$
%number of $w$-selector gates, and of depth $O(\log n)$.
\label{thm:intro-tc-circ}
\end{theorem}
%The techniques for achieving 
To prove the above theorem, 
we need fairly sophisticated and novel techniques.
At a high level, 
to avoid suffering from the super-polylogarithmic depth 
of Asharov et al.~\cite{soda21}, we first construct 
various building blocks that can be regarded as
relaxations of (tight) compaction.
Specifically, by relaxing compaction along several different axes,  
we define several new, intermediate abstractions, 
each of which will play a role in the final construction. 
We show that the relaxed abstractions can be 
realized in sub-logarithmic or logarithmic depth.
We then gradually bootstrap these building blocks into 
stronger ones, and the final tight compaction circuit 
is achieved through multiple steps of bootstrapping.
We defer the details to Section~\ref{sec:roadmap}. 

\medskip
In summary, since both stepping stones require novel 
and fairly sophisticated techniques, 
our final sorting circuit construction  
departs significantly from 
the most closely related prior works~\cite{osortsmallkey,soda21}.
We define numerous new algorithmic abstractions
along the way, some of which  
%some of these new abstractions
may be of independent interest.

%``imperfect'' building blocks that are 
%each ``imperfect'' in incomparable ways.
%We then combine these building blocks and bootstrap 
%into stronger ones. 






\ignore{say there are other challenges besides these two? 
the entire package
departs significantly from the earlier, and is 
novel from the ground up}






==> tcfromlc.tex <==
\section{Tight Compaction from Loose Compaction}

\subsection{Approximate Swapper Circuit}
%\paragraph{Definition.}

\paragraph{Approximate swapper.}
Let $\alpha \in (0, 1)$.
An $(\alpha, n, w)$-approximate swapper 
(also written as $\alpha$-approximate swapper
when $n$ and $w$ are clear from the context)
obtains an input array where
each element is marked with a label that is 
 $\bot$, ${\tt blue}$, or ${\tt red}$.
Let $n_{\rm red}$ and $n_{\rm blue}$
denote the number of red and blue elements, respectively.
The $(\alpha, n, w)$-approximate swapper 
circuit swaps a subset of the ${\tt blue}$
elements with ${\tt red}$ ones and the swapped 
elements receive the label $\bot$.
We call elements marked ${\tt red}$ or ${\tt blue}$
{\it colored} and those marked $\bot$ {\it uncolored}.

Formally, an $(\alpha, n, w)$-approximate swapper 
solves the following problem:
\begin{itemize}[leftmargin=5mm,itemsep=1pt]
\item {\bf Input}:
an input array containing $n$ elements
where each element contains a $w$-bit payload string
and a two-bit metadata label
whose value is chosen
from the set $\{{\tt blue}, {\tt red}, \bot\}$.
Henceforth we assume the first bit of the label
encodes whether the element is colored or not, 
and the second bit of the label
picks a color between ${\tt blue}$ and ${\tt red}$ 
if the element is indeed colored.

\item {\bf Output}:
a {\it legal swap} of the input array such that
at most $n/128 + |n_{\rm red} - n_{\rm blue}|$ 
elements remain colored, where the notion of
a legal swap is defined below.

We say that an output array ${\bf O}$ is a {\it legal swap}
of the input array ${\bf I}$ iff
there exist pairs $(i_1, j_1), (i_2, j_2), \ldots, (i_\ell, j_\ell)$
of indices that are all distinct,
such that for all $k \in [\ell]$, ${\bf I}[i_k]$
and ${\bf I}[j_k]$ are colored and have opposite colors,
and moreover ${\bf O}$ is obtained by swapping
${\bf I}[i_1]$ with ${\bf I}[j_1]$,
swapping ${\bf I}[i_2]$ with ${\bf I}[j_2]$,  $\ldots$, and
swapping ${\bf I}[i_k]$ with ${\bf I}[j_k]$; further, all swapped
elements become uncolored.
%\elaine{this constant matches that of loose compact}
\end{itemize}

\paragraph{Swapper.}
If $\alpha = 0$, i.e., all colored elements are swapped
except for the residual caused by imbalance $|n_{\rm red} - n_{\rm blue}|$,
then we simply call it a {\it swapper}.
Formally, 
an $(0, n, w)$-approximate swapper is also called 
an {\it $(n, w)$-swapper} (or simply {\it swapper} for short).


%\paragraph{Construction.}

%\subsection{$\frac{1}{128}$-Approximate Swapper}
\begin{theorem}[$1/128$-approximate swapper]
There exists a $(1/128, n, w)$-approximate swapper 
circuit containing $O(n)$ generalized boolean gates 
and $O(n)$ number of $w$-selector gates, \elaine{is it w} and of depth 
$O(1)$.
\label{thm:approxswap}
\end{theorem}
\begin{proof}
\elaine{TODO: prove the above, use itc paper}
\end{proof}

\ignore{
\begin{theorem}[$1/\poly \log n$-approximate swapper]
Suppose that there is an 
$(\alpha, n, w)$-lossy loose compaction
circuit with $B_{\rm lc}(n)$
generalized boolean gates and $S_{\rm lc}(n)$ $w$-selector gates,
and of depth $D_{\rm lc}(n)$.
Then, 
for any constant $c > 1$, 
there exists a $(1/\log^c n, n, w)$-approximate swapper 
circuit containing %$O(n)$ 
\elaine{FILL}
generalized boolean gates 
and  \elaine{FILL}
number of $w$-selector gates, and of depth  
\elaine{FILL}.
\end{theorem}
}

\begin{theorem}[Slow swapper]
There exists an $(n, w)$-swapper circuit (henceforth
denoted ${\bf SlowSwap}(\cdot)$) 
with $O(n \log n)$
generalized boolean gates, 
and $O(n \log n)$ $w$-selector gates \elaine{is it w},
and whose depth is $O(\log n)$.
\label{thm:slowswap}
\end{theorem}
\elaine{TO FIX: this requires a pipelined version of AKS? 
in a pipelined fashion, all gates populate the flag first.
}
\begin{proof}
\end{proof}


\subsection{Tight Compaction from Loose Compaction}

\paragraph{Approximate tight compaction.}
Let $\alpha \in (0, 1)$.
An $(\alpha, n, w)$-approximate tight compactor
(also written as $\alpha$-approximate tight compactor
when $n$ and $w$ are clear from the context)
solves the following problem:
given an input array ${\bf I}$ containing $n$ elements, 
each containing  
a $1$-bit key and a $w$-bit payload, 
we want to output 
a permutation (denoted ${\bf O}$) of the input array ${\bf I}$, such that 
at most $\alpha \cdot n$ elements 
in ${\bf O}$
are misplaced  --- here, an element ${\bf O}[i]$ is said
be misplaced iff ${\bf O}[i]$ is marked
with the key $b \in \{0, 1\}$; however, 
the sorted array ${\sf sorted}({\bf I})$
contains the key $1-b$ in position $i$. 



\begin{theorem}[Tight compaction from loose compaction]
Suppose that there is an 
$(\alpha, n, w)$-lossy loose compaction
circuit with $B_{\rm lc}(n)$
generalized boolean gates and $S_{\rm lc}(n)$ $w$-selector gates,
and of depth $D_{\rm lc}(n)$.
%that loosely compacts an input array 
%containing $n$ elements each of bit-width $w$.
Suppose also that there is an $O(1)$-depth 
approximate swapper circuit with
$B_{\rm lsw}(n)$
generalized boolean gates and $S_{\rm lsw}(n)$ $w$-selector gates
for an input array containing $n$ element each of bit-width $w$.
Moreover, suppose that $B_{\rm lc}(n) \geq n$,
$S_{\rm lc}(n) \geq n$,
$B_{\rm lsw}(n) \geq n$, and
$S_{\rm lsw}(n) \geq n$. \elaine{check where 
these conditions are used}

Then, there is a %\elaine{FILL in param}
$(8\alpha, n, w)$-approximate tight compaction circuit  
\elaine{todo: change constant}
with at most
%\elaine{FILL}
$4B_{\rm lsw}(n) + 2B_{\rm lc}(n) + 8S_{\rm lc}(n) + O(n)$
generalized boolean gates, 
and at most
$2S_{\rm lsw}(n) + 4S_{\rm lc}(n) + O(n)$
%$2S_{\rm lsw}(n) + 4S_{\rm lc}(n) + 2n$
number of $w$-selector gates, and 
of depth $8 \log \log n \cdot (D_{\rm lc}(n) + O(1))$. 
\elaine{TODO: change the constant}
\label{thm:tcfromlc}
\end{theorem}

\begin{proof}

For convenience, henceforth we refer to elements with the $0$-key 
as distinguished.
Consider the following algorithm.
\begin{enumerate}[leftmargin=6mm,itemsep=1pt]
\item 
{\it Near-sort.}
\label{step:nearsort}
\item 
{\it Color.}
\elaine{FILL}
Let the outcome be ${\bf X}$. 

Note that at this moment, each element 
is labeled with 3 bits of metadata, one bit of distinguished indicator
and two bits of color-indicator (indicating whether the element is colored,
and if so, which color).
\label{step:mark}

\item 
{\it Swap.}
Call ${\bf Swap}({\bf X}, n)$
%Call an $(1/\log^8 n, n, w + 1)$-approximate-swapper 
%(see Section~\ref{sec:swapper} 
%\elaine{fill, change const}) 
to swap the ${\tt blue}$ elements with ${\tt red}$ elements 
except for a small residual fraction 
(we use here payload of size $w+1$ and not $w$ as 
we also include the color-indicator as part of the payload). 
%Specifically, an $(n, w + 1)$-swapper 
%is defined exactly like a loose swapper but  
%with the requirement that the outcome array must 
%have no colored elements remaining.
\end{enumerate}

\begin{mdframed}
\begin{center}
%{\bf $(1/\log^c n, n, w)$-approximate swapper}
${\bf Swap}({\bf X}, n)$
\end{center}
\begin{itemize}[leftmargin=5mm,itemsep=0pt]
\item {\bf Input:} An array {\bf X} of $m \leq n$ 
elements, each has a $w$-bit payload\footnotemark and a 2-bit label indicating whether the element is colored,
and if so, whether the element is ${\tt blue}$ or ${\tt red}$.
$n$ is the size of the original problem when 
${\bf Swap}$ is first called; the same $n$   
will passed into all recursive 
calls since the recursion will stop when $m \leq n/\log n$.

\item {\bf The algorithm:}
\begin{enumerate}[leftmargin=5mm,itemsep=1pt] %[label=(\alph*)]
\item 
If $m \leq n/\log^c n$, then %\elaine{FILL AKS and return};
return 
\elaine{FILL: don't do anything here, fill in constant c}
%${\bf SlowSwap}({\bf X})$ where ${\bf SlowSwap}$ is described
%in Theorem~\ref{thm:slowswap}; 
else continue with the following steps. 

\item 
%Let $n= |{\bf X}|$; 
Call an $(1/128, m, w)$-loose swapper (see Theorem~\ref{thm:approxswap}) 
on ${\bf X}$ to swap elements of opposite colors 
and uncolor them in the process,
such that at most $1/128$ fraction of resulting array remain colored. 

%Note that the loose swapper treats 
%the two bits of color indicator as metadata
%and each element along with its dummy indicator
%as the payload.
%The loose swapper is parametrized with $n = |{\bf X}|$ and 
\label{step:swap}
\item 
Call an $(1/\log^8 n, m, w+1)$-loose 
compactor (see \elaine{refer}) \elaine{change const}
%(see Section~\ref{sec:})
to compact the outcome of the previous step by a half, 
where the loose compactor treats the colored elements 
as real and the uncolored elements as fillers.
In other words, the loose compactor treats the 1st bit of the color label
as a filler indicator, and treats the 2nd bit of the color label and an 
element's payload string as the payload.
Let the outcome be ${\bf Y}$ whose length is half of ${\bf X}$.
\label{step:compact}
\item 
Recursively call ${\bf Swap}({\bf Y}, n)$, 
and let the outcome be ${\bf Y}'$.
\item 
Reverse the routing decisions made by all selector gates 
during Step~\ref{step:compact} as below.
For every selector gate $g$ in Step~\ref{step:compact}, 
its reverse selector gate denoted $g'$ 
is one that receives a single element as input and outputs two elements; the same control
bit $b$ input to the original gate $g$ 
is used by $g'$ to select which of the output 
receives the input element, and the other one will simply receive the string $0^{w+1}$.
If $g$ selected the first input element to route to the output, then 
in $g'$, the input element is routed to the first output.


In this way, we can reverse-route elements in ${\bf Y}'$ 
to an array (denoted $\widetilde{\bf X}$) of length $|{\bf X}|$, i.e., twice the length
of ${\bf Y}'$.

\label{step:reverse}
\item 
The output ${\bf Z}$ is formed by a performing coordinate-wise 
select operation between ${\bf X}$ and $\widetilde{\bf X}$:
\elaine{TO FIX: this needs to be fixed, some colored 
elements are not propagated by the loose compactor} 
\[
{\bf Z}[i] = 
\begin{cases}
{\bf X}[i] & \text{if ${\bf X}[i]$ is uncolored}\\
\widetilde{\bf X}[i] & \text{o.w.}\\
\end{cases}
\]
%for each $1\leq i \leq |{\bf X}|$, if ${\bf X}[i]$
%is uncolored, let ${\bf R}[i] = {\bf X}[i]$; else
%let 
\ignore{back to the input ${\bf X}$, such that each position 
$i$ receives either a real or a dummy element: if a real element
is received the element ${\bf X}[i]$ is overwritten with the received element;
otherwise the element ${\bf X}[i]$ is unchanged.
Finally, output the result.
}
\label{step:output}
\end{enumerate} 
\item {\bf Output:} The  array {\bf Z}. 
\end{itemize}
\end{mdframed}

\elaine{FILL}



\end{proof}


